Memory Manipulation

We study persuasion that works through memory: a manipulator alters the probabilities with which a Bayesian decision-maker recalls the signals he has received. The decision-maker corrects for the elevated or reduced probabilities of recalling different signals, and this correction disciplines what manipulation can achieve. Manipulation cannot move the average posterior. It backfires on decision-makers with few memories, whose sparse recall is evidence against the favored state, yet it is effective on those with many, who can be led to arbitrarily confident beliefs in the wrong state. It thickens the right tail of the belief distribution and, under Poisson memory, lowers its hazard rate. In a monopoly pricing application, the seller manipulates memory retrieval at high prices, and manipulation in turn raises the optimal price. In a narrative persuasion application, memory manipulation reduces information provision and creates echo chambers.

==> style.tex <==
% Macros File

\usepackage[english]{babel}
\let\circledS\undefined
%\usepackage[adobe-utopia,cal=cmcal]{mathdesign}
\usepackage{amsmath,amsfonts,amsthm,amssymb,mathrsfs, xpatch, dsfont,ushort,sgamevar, float, framed, multirow, array, makecell, comment, url, graphicx, mathtools, fnpct, setspace, pifont,bm,bbm, accents,booktabs,xr,arydshln,pbox}
\usepackage{epstopdf}
\usepackage[a4paper,left=2cm,right=2cm,top=2cm,bottom=2cm]{geometry}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%\usepackage[normalem]{ulem}
\renewcommand{\UrlFont}{\small\tt}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

%\usepackage{lmodern}
\usepackage[final, babel]{microtype}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D\infdivx}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}


\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{titlesec}
\allowdisplaybreaks

\newtheorem{thm}{Theorem}
\usepackage{natbib}
\usepackage[bottom, multiple]{footmisc}

\usepackage{xcolor}
\definecolor{navyblue}{rgb}{0.0, 0.13, 0.28}
\definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
\usepackage{hyperref}
\hypersetup{
	colorlinks=true,
	linkcolor=red,
	filecolor=black,
	citecolor=navyblue,      
	urlcolor=amaranth,
}

\DeclareMathAlphabet{\mathsf}{OT1}{\sfdefault}{m}{n}
\SetMathAlphabet{\mathsf}{bold}{OT1}{\sfdefault}{b}{n}
\usepackage{enumitem}
\newcommand{\argmin}{\arg\!\min}
\newcommand{\argmax}{\arg\!\max}
\renewcommand\qedsymbol{$\blacksquare$}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\usepackage{tocloft}
\newtheorem{propx}{Proposition}
\newtheorem{prop*}{Proposition}[]
\newtheorem{thm*}{Theorem}[]
\newtheorem{claim*}{Claim}[]
\newtheorem{cor*}{Corollary}[]
\newtheorem{ax*}{Axiom}[]
\newtheorem{lem*}{Lemma}[]
\newtheorem{rem*}{Remark}[]
\newtheorem{asp*}{Assumption}[]
\newtheorem{pty*}{Property}[]
\newtheorem{def*}{Definition}[]
\newtheorem{cond*}{Condition}[]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{cond}[thm]{Condition}
\newtheorem{clm}[thm]{Claim}
\newtheorem{defn}[thm]{Definition}
\newtheorem{eg}[thm]{Example}
\newtheorem{remark}[thm]{Remark}
\newtheorem*{propnonumber*}{Proposition}


\newtheorem{aprop}{Proposition}
\renewcommand\theaprop{A\arabic{aprop}}

\usepackage[labelfont=bf]{caption}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{automata,positioning}
\usetikzlibrary{arrows,intersections}
\usetikzlibrary{arrows.meta}
%\usepackage{gensymb}



%\titleformat*{\section}{\Large\bfseries}
%\titleformat*{\subsection}{\large\bfseries}
%\titleformat*{\subsubsection}{\bfseries}
%\titleformat*{\paragraph}{\bfseries}
%\titleformat*{\subparagraph}{\bfseries}

%\let\oldproofname=\proofname
%\renewcommand{\proofname}{\rm\bf{\oldproofname}}
\usepackage{mathptmx}
\newtheorem{example}{Example}
\newenvironment{eg*}
{\pushQED{\qed}\renewcommand{\qedsymbol}{$\blacklozenge$}\examplex}
{\popQED\endexamplex}
\newcommand{\concat}{\hat{~}}
\newcommand{\bp}{{\bf p}}
\newcommand{\vphi}{\varphi}
\newcommand{\ve}{\varepsilon}
\newcommand{\bF}{{\bf F}}
\newcommand{\bP}{{\bf P}}
\newcommand{\gw}{\omega}
\newcommand{\gr}{\rho}
\newcommand{\bt}{{\bf t}}
\newcommand{\bmm}{{\bf m}}
\newcommand{\by}{\bf y}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\hbphi}{\hat{\bphi}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bVar}{{\bf Var}}
\newcommand{\tChi}{\textnormal{Chi}}
\newcommand{\tShi}{\textnormal{Shi}}
\newcommand{\tEi}{\textnormal{Ei}}
\newcommand{\bBZ}{{\mathbb{Z}}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\expo}{ \operatorname{e}}
\newcommand{\gl}{\lambda}
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gd}{\delta}
\newcommand{\gs}{\sigma}
\newcommand{\Gs}{\Sigma}
\newcommand{\gam}{\gamma}
\newcommand{\gk}{\kappa}
\newcommand{\egg}{e.g.,~}
\newcommand{\ie}{i.e.,~}
\usepackage[title, toc]{appendix}
%\setcounter{tocdepth}{2}
\usepackage{xr}


\makeatletter
\renewenvironment{proof}[1][\proofname]{%
	\par\pushQED{\qed}\normalfont%
	\topsep6\p@\@plus6\p@\relax
	\trivlist\item[\hskip\labelsep\bfseries#1\@addpunct{.}]%
	\ignorespaces
}{%
	\popQED\endtrivlist\@endpefalse
}
\makeatother




\newenvironment{myepigraph}
{\par\hfill\itshape
	\begin{tabular}{@{}r@{\hspace{2em}}}} % 2em from the right margin
	{\end{tabular}\par\medskip}


\parskip 1ex
\pgfplotsset{compat=1.14}
\onehalfspacing

